ARACDE: Retrofitting Databases with ABAC using External Authorization Engines

This paper proposes a methodology for decoupling the authorization logic of a relational database from its core data management engine, enabling specification of advanced access control policies with minimal changes to the code base. Our decoupled authorization architecture, which we call ARCADE, externalizes access request resolution to a formally verifiable policy engine (e.g., Cedar), while the database itself enforces those decisions. We showcase the capabilities of ARCADE on two widely popular open-source databases, namely MySQL and PostgreSQL. Purpose built lightweight plugins add an Attribute-based Access Control (ABAC) layer that augments the native discretionary and role-based access control capabilities of these databases. ARCADE supports highly expressive policies using attributes of subjects, objects, and the environment, and the use of Cedar enables easy auditing and verification of the specified policies. It follows a design principle that mitigates potential risks in segregating authorization from the database core through low footprint, network isolation, and a policy composition methodology that does not negate any native authorization. Experiments on TPC-C, TPC-B, and a custom workload show that ARCADE incurs negligible performance overhead, for instance, less than 3.9% throughput penalty for MySQL (1.3% for PostgreSQL) on industry standard TPC-C benchmark.

==> Makefile <==
LATEXFLAGS = -file-line-error-style -halt-on-error -shell-escape

all:
	pdflatex $(LATEXFLAGS) main
	biber main
	pdflatex $(LATEXFLAGS) main
	pdflatex $(LATEXFLAGS) main
	@echo ""
	@echo "=== Build Summary ==="
	@pages=$$(pdfinfo main.pdf 2>/dev/null | awk '/^Pages:/ {print $$2}'); \
		echo "Pages: $${pages:-?}"
	@warning_count=$$(grep -c 'Warning' main.blg 2>/dev/null); \
		warning_count=$${warning_count:-0}; \
		if [ "$$warning_count" -gt 0 ]; then \
			echo "$$warning_count biber warnings (see main.blg)"; \
		fi
	@grep 'Font Warning' main.log 2>/dev/null | sort -u || true
	@overfull_count=$$(grep -c 'Overfull' main.log 2>/dev/null || echo 0); \
		echo "$$overfull_count overfull hbox warnings"
	@echo "Output: main.pdf"

# Check that all fonts are embedded (required for ACM CCS submission)
fontcheck:
	@echo "=== Font Embedding Check ==="
	@pdffonts main.pdf | head -1
	@pdffonts main.pdf | tail -n +2 | while read line; do \
		echo "$$line"; \
	done
	@echo ""
	@if pdffonts main.pdf | tail -n +2 | grep -q ' no '; then \
		echo "WARNING: Some fonts are NOT embedded!"; \
		pdffonts main.pdf | grep ' no '; \
	else \
		echo "OK: All fonts embedded."; \
	fi

# --- Reviewer diff (latexdiff) ---------------------------------------------
# Renders the inline textual diff against a baseline git revision: additions
# are underlined in blue, deletions struck through in red. The "new" side is
# the current working tree (uncommitted edits included), so no commit is
# needed. Override the baseline with:  make diff DIFFBASE=<rev>
DIFFBASE ?= submission-v1
DIFFDIR   = .diffbuild

diff:
	@command -v latexdiff >/dev/null || { echo "error: latexdiff not found (install TeX Live)"; exit 1; }
	@command -v latexpand >/dev/null || { echo "error: latexpand not found (install TeX Live)"; exit 1; }
	${RM} -r $(DIFFDIR)
	mkdir -p $(DIFFDIR)/old $(DIFFDIR)/new
	git archive $(DIFFBASE) | tar -x -C $(DIFFDIR)/old
	newrev=$$(git stash create); git archive $${newrev:-HEAD} | tar -x -C $(DIFFDIR)/new
	cd $(DIFFDIR)/old && latexpand main.tex > ../old-flat.tex 2>/dev/null
	cd $(DIFFDIR)/new && latexpand main.tex > ../new-flat.tex 2>/dev/null
	cd $(DIFFDIR) && latexdiff old-flat.tex new-flat.tex > new/main-diff.tex
	cd $(DIFFDIR)/new && pdflatex $(LATEXFLAGS) main-diff && biber main-diff && \
		pdflatex $(LATEXFLAGS) main-diff && pdflatex $(LATEXFLAGS) main-diff
	cp $(DIFFDIR)/new/main-diff.pdf main-diff.pdf
	@echo ""
	@echo "=== Diff Summary (baseline $(DIFFBASE)) ==="
	@pages=$$(pdfinfo main-diff.pdf 2>/dev/null | awk '/^Pages:/ {print $$2}'); \
		echo "Pages: $${pages:-?}"
	@echo "Output: main-diff.pdf"

clean:
	${RM} *~ *.aux *.log *.dvi *.ps main.pdf body.tmp head.tmp *.bbl *.blg *.out *.bak final-paper.pdf
	${RM} main-diff.pdf
	${RM} -r _minted-paper $(DIFFDIR)

.PHONY: all clean fontcheck diff

